Stretching Demi-Bits and Nondeterministic-Secure Pseudorandomness

We develop the theory of cryptographic nondeterministic-secure pseudorandomness beyond the point reached by Rudich's original work (Rudich 1997), and apply it to draw new consequences in average-case complexity and proof complexity. Specifically, we show the following: *Demi-bit stretch*: Super-bits and demi-bits are variants of cryptographic pseudorandom generators which are secure against nondeterministic statistical tests (Rudich 1997). They were introduced to rule out certain approaches to proving strong complexity lower bounds beyond the limitations set out by the Natural Proofs barrier (Rudich and Razborov 1997). Whether demi-bits are stretchable at all had been an open problem since their introduction. We answer this question affirmatively by showing that: every demi-bit $b:\{0,1\}^n\to \{0,1\}^{n+1}$ can be stretched into sublinear many demi-bits $b':\{0,1\}^{n}\to \{0,1\}^{n+n^{c}}$, for every constant $0<c<1$. >>> see rest of abstract in paper.

==> 0.2.acknowledgements.tex <==
%\section*{Acknowledgements}
\addcontentsline{toc}{section}{Acknowledgements}
\forceindent
I shall give deep thanks to my thesis supervisor Prof Iddo Tzameret for his meticulous and remarkable supervision and guidance, and deep thanks to my friend Yufeng Li for his timely assistance with many \LaTeX{} related issues.
%
I shall also give thanks to Dr Iain Phillips for providing helpful midway feedback and to Prof Rahul Santhanam and Dr J{\'{a}}n Pich for discussion in the mid-course.
%
Without their help, the completion of this project would have been impossible.


